A New Class of Fully Discrete Sparse Fourier Transforms: Faster Stable Implementations with Guarantees

In this paper we consider Sparse Fourier Transform (SFT) algorithms for approximately computing the best $s$-term approximation of the Discrete Fourier Transform (DFT) $\mathbf{\hat{f}} \in \mathbb{C}^N$ of any given input vector $\mathbf{f} \in \mathbb{C}^N$ in just $\left( s \log N\right)^{\mathcal{O}(1)}$-time using only a similarly small number of entries of $\mathbf{f}$. In particular, we present a deterministic SFT algorithm which is guaranteed to always recover a near best $s$-term approximation of the DFT of any given input vector $\mathbf{f} \in \mathbb{C}^N$ in $\mathcal{O} \left( s^2 \log ^{\frac{11}{2}} (N) \right)$-time. Unlike previous deterministic results of this kind, our deterministic result holds for both arbitrary vectors $\mathbf{f} \in \mathbb{C}^N$ and vector lengths $N$. In addition to these deterministic SFT results, we also develop several new publicly available randomized SFT implementations for approximately computing $\mathbf{\hat{f}}$ from $\mathbf{f}$ using the same general techniques. The best of these new implementations is shown to outperform existing discrete sparse Fourier transform methods with respect to both runtime and noise robustness for large vector lengths $N$.

==> Algorithm1.tex <==
\begin{algorithm}
\label{Alg1}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
    \Input{Signal pointer $f$, sparsity $s$, choose $\ensuremath{\tau\in\left(0,\frac{1}{\sqrt{2\pi}}\right)}$,
$\alpha\in\left[1,\frac{N}{\sqrt{\ln N}}\right]$, $\ensuremath{\beta\in\left(0,\alpha\sqrt{\frac{\ln\left(1/\tau\sqrt{2\pi}\right)}{2}}~\right]}$}
    \Output{$\widehat{R}^s$, a sparse representation of $\widehat{f}$}
    Initialize $\widehat{R}, \widehat{R}^s \leftarrow\emptyset$
    
    Set $c_1 = \frac{\beta \sqrt{\ln N}}{N}$, $c_2 = \frac{\alpha \sqrt{\ln N}}{2}$
    
    Compute the sampling scheme of SFT
    
    \For{$k$ from $1$ to $c_2$}{
        $q = -\big\lceil \frac{N}{2}\big\rceil + 1 + k\big\lceil \frac{N}{\alpha \sqrt{\ln N}} \big\rceil$  \\
        Shift filter function $g$ in Fourier space by $q$ and define the new function as $\tilde{g}$, i.e. $\tilde{g}(x) = g(x)\cdot e^{\i q(x)}$ \\
        \For{each point $x$ in sampling scheme}{
            Compute the value of $(\tilde{g}\ast f)$ at $x$\\
        }
        Apply deterministic SFT algorithm to find $s$ significant frequencies $\omega$ and their coefficients $C_{\omega}$ in the current effective support of function $\tilde{g}$, that is $[q - \big\lceil\frac{N}{\alpha \sqrt{\ln N}}\big\rceil, q + \big\lceil\frac{N}{\alpha \sqrt{\ln N}}\big\rceil]$, store the all the pairs $(\omega, C_{\omega})$ in $R_{temp}$\\
        \For{all $(\omega, C_{\omega})$ pairs in $R_{temp}$}{
            $\widehat{R} \leftarrow (\omega, \tilde{C}_{\omega})$, where $\tilde{C}_{\omega} = \sqrt{2\pi}e^{\frac{{c_1}^2 (q - \omega)^2}{2}}C_{\omega}$
        }
    }
    
    Choose $s$ pairs of $(\omega, \tilde{C}_{\omega})$ in $\widehat{R}$ which has largest magnitude $\tilde{C}_{\omega}$ and put them in $\widehat{R}^s$\\
    
    Return $\widehat{R}^s$
    
    
        
    \caption{Discrete SFT algorithms}
\end{algorithm}

We display the general idea of discrete SFT in Algorithm 1. The periodic Gaussian function $g$ is used as a filter function. The algorithm works by shifting the filter function $g$ for several times in Fourier space until it cover the whole bandwidth. For fixed filter function $g$, we apply the GFFT algorithm to find the $s$ most significant frequencies of $g\ast f$. At the very end, we collect all the frequencies and coefficients we found and select $s$ frequencies which has the largest magnitude. 

The idea of Algorithm 1 is simple but it is not a fully discrete algorithm. Remember that in discrete case we only have $N$ equally spaced samples of the signal function $f$, which means the convolution in line 8 cannot be computed exactly. Seems like the best option we have under the discrete setting is to use discrete convolution to approximate line 8. However, this may cause two problems. The first is that the value of $g\ast f$ is contaminated by the numerical error between continuous and discrete convolution, which may cause some robustness problems in the recovery part. The second is that the computational cost for discrete convolution is $\mathcal{O}(N)$ for each point of the function $g\ast f$, which is too expensive. In the rest part of this section, we prove that by choosing the parameters in $g$ carefully, we can approximate $g\ast f$ in arbitrary high accuracy by only using a very small portion of the terms in the discrete convolution. 










